C11Tester: A Race Detector for C/C++ Atomics Technical Report

Writing correct concurrent code that uses atomics under the C/C++ memory model is extremely difficult. We present C11Tester, a race detector for the C/C++ memory model that can explore executions in a larger fragment of the C/C++ memory model than previous race detector tools. Relative to previous work, C11Tester's larger fragment includes behaviors that are exhibited by ARM processors. C11Tester uses a new constraint-based algorithm to implement modification order that is optimized to allow C11Tester to make decisions in terms of application-visible behaviors. We evaluate C11Tester on several benchmark applications, and compare C11Tester's performance to both tsan11rec, the state of the art tool that controls scheduling for C/C++; and tsan11, the state of the art tool that does not control scheduling.

==> makefile <==
TECHREPORT = techreport
PAPER = paper
ABSTRACT = extended-abstract
#AE = artifact-appendix
TEX = $(wildcard *.tex)
BIB = all.bib
FIGS = $(wildcard figures/*.pdf figures/*.png graphs/*.pdf graphs/*.png)
PACKAGE=acmart
CURRFOLDER=revision1.notechreport
OLDFOLDER=submitted.asplos/notechreport

.PHONY: all clean

all: $(PAPER).pdf

$(TECHREPORT).pdf: $(TEX) $(BIB) $(FIGS) $(PACKAGE).cls
	echo $(FIGS)
	pdflatex $(TECHREPORT)
	bibtex $(TECHREPORT)
	pdflatex $(TECHREPORT)
	pdflatex $(TECHREPORT)

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS) $(PACKAGE).cls
	echo $(FIGS)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

$(ABSTRACT).pdf: $(TEX) $(BIB) $(FIGS) $(PACKAGE).cls
	pdflatex $(ABSTRACT)
	bibtex $(ABSTRACT)
	bibtex $(ABSTRACT)
	pdflatex $(ABSTRACT)
	pdflatex $(ABSTRACT)

#$(AE).pdf: $(TEX) $(BIB) $(FIGS) $(PACKAGE).cls
#	pdflatex $(AE)
#	bibtex $(AE)
#	bibtex $(AE)
#	pdflatex $(AE)
#	pdflatex $(AE)

diff:
	[ -d diff ] || mkdir diff
	latexdiff --packages=hyperref --exclude-textcmd="section" $(OLDFOLDER)/paper.tex $(CURRFOLDER)/paper.tex > diff/paper.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/abstract.tex $(CURRFOLDER)/abstract.tex > diff/abstract.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/appendix.tex $(CURRFOLDER)/appendix.tex > diff/appendix.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/conclusion.tex $(CURRFOLDER)/conclusion.tex > diff/conclusion.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/eval.tex $(CURRFOLDER)/eval.tex > diff/eval.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/intro.tex $(CURRFOLDER)/intro.tex > diff/intro.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/implementation.tex $(CURRFOLDER)/implementation.tex > diff/implementation.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/memorymodel.tex $(CURRFOLDER)/memorymodel.tex > diff/memorymodel.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/proof.tex $(CURRFOLDER)/proof.tex > diff/proof.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/related.tex $(CURRFOLDER)/related.tex > diff/related.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/semantics.tex $(CURRFOLDER)/semantics.tex > diff/semantics.tex
	latexdiff --exclude-textcmd="section" $(OLDFOLDER)/technical.tex $(CURRFOLDER)/technical.tex > diff/technical.tex
	cp ./macros.tex diff/
	cp ./acmart.* diff/
	cp ./ACM-Reference-Format.* diff/
	cp ./*.cc diff/
	cp ./confstrs-* diff/
	cp ./makefile diff/
	cp ./paper.bib ./all.bib diff/
	cp -r ./figures ./plots diff/
	cd ./diff; touch artifact-appendix.tex; make diffpdf

spell:
	@for i in *.tex; \
	do if [ $$i != "paper.tex" ]; then aspell -c $$i -p ./spell.lst; fi;\
	done

clean:
	rm -f *.aux *.bbl *.blg *.log *.out $(PAPER).pdf $(ABSTRACT).pdf $(TECHREPORT).pdf

